Automated question generation and question answering from Turkish texts

While exam-style questions are a fundamental educational tool serving a variety of purposes, manual construction of questions is a complex process that requires training, experience and resources. Automatic question generation (QG) techniques can be utilized to satisfy the need for a continuous supply of new questions by streamlining their generation. However, compared to automatic question answering (QA), QG is a more challenging task. In this work, we fine-tune a multilingual T5 (mT5) transformer in a multi-task setting for QA, QG and answer extraction tasks using Turkish QA datasets. To the best of our knowledge, this is the first academic work that performs automated text-to-text question generation from Turkish texts. Experimental evaluations show that the proposed multi-task setting achieves state-of-the-art Turkish question answering and question generation performance on TQuADv1, TQuADv2 datasets and XQuAD Turkish split. The source code and the pre-trained models are available at https://github.com/obss/turkish-question-generation.

==> old_bib.tex <==
\begin{thebibliography}{31}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Yue et~al.(2020)Yue, Zhang, Yao, Lin, and Sun]{yue2020cliniqg4qa}
Xiang Yue, Xinliang~Frederick Zhang, Ziyu Yao, Simon Lin, and Huan Sun.
\newblock Cliniqg4qa: Generating diverse questions for domain adaptation of
  clinical question answering.
\newblock \emph{arXiv preprint arXiv:2010.16021}, 2020.

\bibitem[Mitkov et~al.(2003)]{mitkov2003computer}
Ruslan Mitkov et~al.
\newblock Computer-aided generation of multiple-choice tests.
\newblock In \emph{Proceedings of the HLT-NAACL 03 workshop on Building
  educational applications using natural language processing}, pages 17--22,
  2003.

\bibitem[Heilman and Smith(2010)]{heilman2010good}
Michael Heilman and Noah~A Smith.
\newblock Good question! statistical ranking for question generation.
\newblock In \emph{Human Language Technologies: The 2010 Annual Conference of
  the North American Chapter of the Association for Computational Linguistics},
  pages 609--617, 2010.

\bibitem[Soleymanzadeh(2017)]{soleymanzadeh2017domain}
Katira Soleymanzadeh.
\newblock Domain specific automatic question generation from text.
\newblock In \emph{Proceedings of ACL 2017, Student Research Workshop}, pages
  82--88, 2017.

\bibitem[Du et~al.(2017)Du, Shao, and Cardie]{du2017learning}
Xinya Du, Junru Shao, and Claire Cardie.
\newblock Learning to ask: Neural question generation for reading
  comprehension.
\newblock In \emph{Proceedings of the 55th Annual Meeting of the Association
  for Computational Linguistics (Volume 1: Long Papers)}, pages 1342--1352,
  2017.

\bibitem[Hochreiter and Schmidhuber(1997)]{hochreiter1997long}
Sepp Hochreiter and J{\"u}rgen Schmidhuber.
\newblock Long short-term memory.
\newblock \emph{Neural computation}, 9\penalty0 (8):\penalty0 1735--1780, 1997.

\bibitem[Zhou et~al.(2017)Zhou, Yang, Wei, Tan, Bao, and Zhou]{zhou2017neural}
Qingyu Zhou, Nan Yang, Furu Wei, Chuanqi Tan, Hangbo Bao et al.
\newblock Neural question generation from text: A preliminary study.
\newblock In \emph{National CCF Conference on Natural Language Processing and
  Chinese Computing}, pages 662--671. Springer, 2017.

\bibitem[Zhao et~al.(2018)Zhao, Ni, Ding, and Ke]{zhao2018paragraph}
Yao Zhao, Xiaochuan Ni, Yuanyuan Ding, and Qifa Ke.
\newblock Paragraph-level neural question generation with maxout pointer and
  gated self-attention networks.
\newblock In \emph{Proceedings of the 2018 Conference on Empirical Methods in
  Natural Language Processing}, pages 3901--3910, 2018.

\bibitem[Duan et~al.(2017)Duan, Tang, Chen, and Zhou]{duan2017question}
Nan Duan, Duyu Tang, Peng Chen, and Ming Zhou.
\newblock Question generation for question answering.
\newblock In \emph{Proceedings of the 2017 Conference on Empirical Methods in
  Natural Language Processing}, pages 866--874, 2017.

\bibitem[Kim et~al.(2019)Kim, Lee, Shin, and Jung]{kim2019improving}
Yanghoon Kim, Hwanhee Lee, Joongbo Shin, and Kyomin Jung.
\newblock Improving neural question generation using answer separation.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, volume~33, pages 6602--6609, 2019.

\bibitem[Sun et~al.(2018{\natexlab{a}})Sun, Lyu, He, Ma, and
  Wang]{sun2018answer}
Jing Sun, Xingwu and~Liu, Yajuan Lyu, Wei He, Yanjun Ma et al.
\newblock Answer-focused and position-aware neural question generation.
\newblock In \emph{Proceedings of the 2018 Conference on Empirical Methods in
  Natural Language Processing}, pages 3930--3939, 2018{\natexlab{a}}.

\bibitem[Tuan et~al.(2020)Tuan, Shah, and Barzilay]{tuan2020capturing}
Luu~Anh Tuan, Darsh Shah, and Regina Barzilay.
\newblock Capturing greater context for question generation.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, volume~34, pages 9065--9072, 2020.

\bibitem[Kriangchaivech and Wangperawong(2019)]{kriangchaivech2019question}
Kettip Kriangchaivech and Artit Wangperawong.
\newblock Question generation by transformers.
\newblock \emph{arXiv preprint arXiv:1909.05017}, 2019.

\bibitem[Chan and Fan(2019)]{chan2019recurrent}
Ying-Hong Chan and Yao-Chung Fan.
\newblock A recurrent bert-based model for question generation.
\newblock In \emph{Proceedings of the 2nd Workshop on Machine Reading for
  Question Answering}, pages 154--162, 2019.

\bibitem[Lopez et~al.(2020)Lopez, Cruz, Cruz, and Cheng]{lopez2020transformer}
Luis~Enrico Lopez, Diane~Kathryn Cruz, Jan Christian~Blaise Cruz, and Charibeth
  Cheng.
\newblock Transformer-based end-to-end question generation.
\newblock \emph{arXiv preprint arXiv:2005.01107}, 2020.

\bibitem[Xue et~al.(2020)Xue, Constant, Roberts, Kale, Al-Rfou, Siddhant,
  Barua, and Raffel]{xue2020mt5}
Linting Xue, Noah Constant, Adam Roberts, Mihir Kale, Rami Al-Rfou et al.
\newblock mt5: A massively multilingual pre-trained text-to-text transformer.
\newblock \emph{arXiv e-prints}, pages arXiv--2010, 2020.

\bibitem[Raffel et~al.(2019)Raffel, Shazeer, Roberts, Lee, Narang, Matena,
  Zhou, Li, and Liu]{raffel2019exploring}
Colin Raffel, Noam Shazeer, Adam Roberts, Katherine Lee, Sharan Narang et al.
\newblock Exploring the limits of transfer learning with a unified text-to-text
  transformer.
\newblock \emph{arXiv preprint arXiv:1910.10683}, 2019.

\bibitem[Raffel et~al.(2020)Raffel, Shazeer, Roberts, Lee, Narang, Matena,
  Zhou, Li, and Liu]{raffel2020exploring}
Colin Raffel, Noam Shazeer, Adam Roberts, Katherine Lee, Sharan Narang et al.
\newblock Exploring the limits of transfer learning with a unified text-to-text
  transformer.
\newblock \emph{Journal of Machine Learning Research}, 21:\penalty0 1--67,
  2020.

\bibitem[Rajpurkar et~al.(2016)Rajpurkar, Zhang, Lopyrev, and
  Liang]{rajpurkar2016squad}
Pranav Rajpurkar, Jian Zhang, Konstantin Lopyrev, and Percy Liang.
\newblock Squad: 100, 000+ questions for machine comprehension of text.
\newblock In \emph{EMNLP}, 2016.

\bibitem[Sun et~al.(2018{\natexlab{b}})Sun, Liu, Lyu, He, Ma, and
  Wang]{sun-etal-2018-answer}
Xingwu Sun, Jing Liu, Yajuan Lyu, Wei He, Yanjun Ma et al.
\newblock Answer-focused and position-aware neural question generation.
\newblock In \emph{Proceedings of the 2018 Conference on Empirical Methods in
  Natural Language Processing}, pages 3930--3939, Brussels, Belgium,
  October-November 2018{\natexlab{b}}. Association for Computational
  Linguistics.
\newblock \doi{10.18653/v1/D18-1427}.
\newblock URL \url{https://aclanthology.org/D18-1427}.

\bibitem[Wolf et~al.(2020)Wolf, Debut, Sanh, Chaumond, Delangue, Moi, Cistac,
  Rault, Louf, Funtowicz, Davison, Shleifer, von Platen, Ma, Jernite, Plu, Xu,
  Scao, Gugger, Drame, Lhoest, and Rush]{wolf-etal-2020-transformers}
Thomas Wolf, Lysandre Debut, Victor Sanh, Julien Chaumond, Clement Delangue et al.
\newblock Transformers: State-of-the-art natural language processing.
\newblock In \emph{Proceedings of the 2020 Conference on Empirical Methods in
  Natural Language Processing: System Demonstrations}, pages 38--45, Online,
  October 2020. Association for Computational Linguistics.
\newblock URL \url{https://www.aclweb.org/anthology/2020.emnlp-demos.6}.

\bibitem[Paszke et~al.(2019)Paszke, Gross, Massa, Lerer, Bradbury, Chanan,
  Killeen, Lin, Gimelshein, Antiga, et~al.]{paszke2019pytorch}
Adam Paszke, Sam Gross, Francisco Massa, Adam Lerer, James Bradbury et al.
\newblock Pytorch: An imperative style, high-performance deep learning library.
\newblock In \emph{NeurIPS}, 2019.

\bibitem[TQuAD(2018)]{tquad2018}
TQuAD.
\newblock Turkish question answering dataset.
\newblock https://github.com/TQuad/turkish-nlp-qa-dataset, 2018.

\bibitem{tquadextended2021}
Fatih Soygazi, Okan Çiftçi, Uğurcan Kök, and Soner Cengiz.
\newblock Thquad: Turkish historic question answering dataset for reading
  comprehension.
\newblock In {\em 2021 6th International Conference on Computer Science and
  Engineering (UBMK)}, pages 215--220, 2021.

\bibitem[Artetxe et~al.(2019)Artetxe, Ruder, and Yogatama]{artetxe2019cross}
Mikel Artetxe, Sebastian Ruder, and Dani Yogatama.
\newblock On the cross-lingual transferability of monolingual representations.
\newblock \emph{arXiv preprint arXiv:1910.11856}, 2019.

\bibitem[Amidei et~al.(2018)Amidei, Piwek, and Willis]{amidei2018evaluation}
Jacopo Amidei, Paul Piwek, and Alistair Willis.
\newblock Evaluation methodologies in automatic question generation 2013-2018.
\newblock 2018.

\bibitem[Papineni et~al.(2002)Papineni, Roukos, Ward, and
  Zhu]{papineni2002bleu}
Kishore Papineni, Salim Roukos, Todd Ward, and Wei-Jing Zhu.
\newblock Bleu: a method for automatic evaluation of machine translation.
\newblock In \emph{Proceedings of the 40th annual meeting of the Association
  for Computational Linguistics}, pages 311--318, 2002.

\bibitem[Banerjee and Lavie(2005)]{banerjee2005meteor}
Satanjeev Banerjee and Alon Lavie.
\newblock Meteor: An automatic metric for mt evaluation with improved
  correlation with human judgments.
\newblock In \emph{Proceedings of the acl workshop on intrinsic and extrinsic
  evaluation measures for machine translation and/or summarization}, pages
  65--72, 2005.

\bibitem[Lin(2004)]{lin2004rouge}
Chin-Yew Lin.
\newblock Rouge: A package for automatic evaluation of summaries.
\newblock In \emph{Text summarization branches out}, pages 74--81, 2004.

\bibitem[Devlin et~al.(2018)Devlin, Chang, Lee, and Toutanova]{devlin2018bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language
  understanding.
\newblock \emph{arXiv preprint arXiv:1810.04805}, 2018.

\bibitem[Schweter(2020)]{stefan_schweter_2020_3770924}
Stefan Schweter.
\newblock Berturk - bert models for turkish, April 2020.
\newblock URL \url{https://doi.org/10.5281/zenodo.3770924}.

\end{thebibliography}
